SaFARi: State-Space Models for Frame-Agnostic Representation

State-Space Models (SSMs) have re-emerged as a powerful tool for online function approximation, and as the backbone of machine learning models for long-range dependent data. However, to date, only a few polynomial bases have been explored for this purpose, and the state-of-the-art implementations were built upon the best of a few limited options. In this paper, we present a generalized method for building an SSM with any frame or basis, rather than being restricted to polynomials. This framework encompasses the approach known as HiPPO, but also permits an infinite diversity of other possible "species" within the SSM architecture. We dub this approach SaFARi: SSMs for Frame-Agnostic Representation.

==> Figures/daubechies/daubframe.tex <==
% \documentclass[tikz]{standalone}

% \usepackage{tikz}
% \usepackage{pgfplots}
% \usepackage{pgffor}
% \usepackage{filecontents}
% \usepackage{xcolor}
% \usetikzlibrary{pgfplots.groupplots}
% \pgfplotsset{compat=newest}
% \usepgfplotslibrary{colorbrewer}
% \usetikzlibrary{calc}
% \usetikzlibrary{decorations.pathreplacing,calligraphy}

% \begin{document} 

\begin{tikzpicture}
\tikzstyle{every node}=[font=\Large]
\begin{groupplot}[
    group style={
        group name=myplots,
        group size=1 by 12,
        vertical sep=1mm
    },
    width=15cm,
    height=2cm,
    enlargelimits=false,
    axis line style={draw=none},
    tick style={draw=none},
    xtick=\empty, ytick=\empty,
    cycle list/Dark2,
    ] 
\pgfplotsforeachungrouped \col in {1,...,12}
{
    \edef\tmp{
    \noexpand\nextgroupplot
    \noexpand\addplot+ [smooth,thick,blue!50!black] table     [col sep=comma, x=x, y index=\col] {Figures/daubechies/Daubechies_frame.csv};
    }\tmp
}
\end{groupplot}

\node (title) at ($(myplots c1r1.center)+(0,1cm)$) {Daubechies-22 Wavelet Frame};

\draw [thick, decorate,decoration={calligraphic brace,mirror,amplitude=5pt,raise=5pt}]
(myplots c1r7.north west) -- (myplots c1r12.south west) node [midway,left=10pt]{$\psi_2$};

\draw [thick, decorate,decoration={calligraphic brace,mirror,amplitude=5pt,raise=5pt}]
(myplots c1r4.north west) -- (myplots c1r6.south west) node [midway,left=10pt]{$\psi_1$};

\draw [thick, decorate,decoration={calligraphic brace,mirror,amplitude=5pt,raise=5pt}]
(myplots c1r1.north west) -- (myplots c1r3.south west) node [midway,left=10pt]{$\phi_0$};

\begin{axis}[
    title={Scaled-WaLRUS $A$ Matrix},
    name=axis2, 
    anchor=west, 
    at={(myplots c1r6.east)},  
    xshift=1cm,
    height=8cm,
    width=8cm,
    point meta min=-60,
    point meta max=60,
    enlargelimits=false,
    % axis line style={draw=none},
    tick style={draw=none},
    xtick=\empty, ytick=\empty,
    colormap/PuOr,
    y dir=reverse,
    mesh/ordering=y varies,
    axis on top,
]   
    \addplot [matrix plot*, point meta=explicit] table [meta index=2] {Figures/daubechies/AdaubS.dat};

\end{axis}

\begin{axis}[
    title={Translated-WaLRUS $A$ Matrix},
    name=axis3, 
    anchor=west, 
    at={(axis2.east)},  
    xshift=1cm,
    height=8cm,
    width=8cm,
    point meta min=-60,
    point meta max=60,
    % axis line style={draw=none},
    tick style={draw=none},
    enlargelimits=false,
    xtick=\empty, ytick=\empty,
    colormap/PuOr,
    y dir=reverse,
    mesh/ordering=y varies,
    axis on top,
]     
    \addplot [matrix plot*, point meta=explicit] table [meta index=2]{Figures/daubechies/AdaubT.dat}; 
\end{axis}

\begin{axis}[name=cbar, anchor=west, 
    at={(axis3.east)},
    colorbar,     
    height=8cm,
    width=2cm,
    point meta min=-60,
    point meta max=60,
    % xshift=.25cm,
    axis line style={draw=none},
    tick style={draw=none},
    axis on top,
    xtick=\empty, ytick=\empty,
    colormap/PuOr,]
    \addplot [draw=none] coordinates {(0,0)};
\end{axis}

\end{tikzpicture}

% \end{document}

==> Figures/intro-demo/introfigure.tikz.tex <==
\begin{tikzpicture}
  \begin{groupplot}[
  group style={group name=myplots, 
  group size=2 by 2, 
  horizontal sep=1.5cm,
  vertical sep=1.25cm},
  height=5cm, width=5.5cm,
  ]

  %%% signal plot
  \nextgroupplot[cycle list name=mylist0,
    xlabel=$t$, ylabel=$u(t)$,
    xmin=-1, xmax=1]

  \addplot+
  table [x=t, y expr={100*\thisrow{sig}}, col sep=comma] 
  {Figures/intro-demo/results/signals.csv};
    
  \addplot+
  table [x=t, y expr={100*\thisrow{sig_clean}}, col sep=comma] 
  {Figures/intro-demo/results/signals.csv};

  \draw[dashed] (-0.4,0 |- current axis.south) -- (-0.4,0 |- current axis.north);
  \draw[dashed] (-0.22,0 |- current axis.south) -- (-0.22,0 |- current axis.north);
  \draw[dashed] (-0.1,0 |- current axis.south) -- (-0.1,0 |- current axis.north);
  \draw[dashed] (0.38,0 |- current axis.south) -- (0.38,0 |- current axis.north);
  \draw[dashed] (0.5,0 |- current axis.south) -- (0.5,0 |- current axis.north);



  %%% MSE from top-K approximation
  \nextgroupplot[cycle list name=mylist1,
    xmode=log, ymode=log,
    xlabel=$\log(K)$, ylabel=$\log(\mathrm{MSE})$,
    legend pos=south west,
    log number format basis/.code 2 args={${\pgfmathprintnumber{#2}}$},
    ]
    
  \addplot+
  table [x=K, y=leg_mse, col sep=comma] 
  {Figures/intro-demo/results/errors.csv};
  \addlegendentry{Leg.}

  \addplot+
  table [x=K, y=fou_mse, col sep=comma] 
  {Figures/intro-demo/results/errors.csv};
  \addlegendentry{Fou.}

  \addplot+
  table [x=K, y=dwt_mse, col sep=comma] 
  {Figures/intro-demo/results/errors.csv};
  \addlegendentry{Wav.}


  %%% top wavelet coeffs
  \nextgroupplot[xlabel={$t$}, ylabel={$j$}, xmin=-1, xmax=1]
  \addplot[scatter,only marks]
  table [x=u, y=s, col sep=comma] 
  {Figures/intro-demo/results/dwt_locations.csv};

  \draw[dashed] (-0.4,0 |- current axis.south) -- (-0.4,0 |- current axis.north);
  \draw[dashed] (-0.22,0 |- current axis.south) -- (-0.22,0 |- current axis.north);
  \draw[dashed] (-0.1,0 |- current axis.south) -- (-0.1,0 |- current axis.north);
  \draw[dashed] (0.38,0 |- current axis.south) -- (0.38,0 |- current axis.north);
  \draw[dashed] (0.5,0 |- current axis.south) -- (0.5,0 |- current axis.north);



  
  \nextgroupplot[]
  \addplot coordinates {(0,2) (1,1) (2,1)};
    
  \end{groupplot}

  \foreach \p/\l in {c1r1/a, c2r1/b, c1r2/c, c2r2/d} {
  \node[anchor=north east] 
  at (myplots \p.north east) {\textbf{(\l)}};
  };
\end{tikzpicture}
